Characterizing the FRB host galaxy population and its connection to transients in the local and extragalactic Universe

We present the localization and host galaxies of one repeating and two apparently non-repeating Fast Radio Bursts. FRB20180301A was detected and localized with the Karl G. Jansky Very Large Array to a star-forming galaxy at $z=0.3304$. FRB20191228A, and FRB20200906A were detected and localized by the Australian Square Kilometre Array Pathfinder to host galaxies at $z=0.2430$ and $z=0.3688$, respectively. We combine these with 13 other well-localized FRBs in the literature, and analyze the host galaxy properties. We find no significant differences in the host properties of repeating and apparently non-repeating FRBs. FRB hosts are moderately star-forming, with masses slightly offset from the star-forming main-sequence. Star formation and low-ionization nuclear emission-line region (LINER) emission are major sources of ionization in FRB host galaxies, with the former dominant in repeating FRB hosts. FRB hosts do not track stellar mass and star formation as seen in field galaxies (more than 95% confidence). FRBs are rare in massive red galaxies, suggesting that progenitor formation channels are not solely dominated by delayed channels which lag star formation by Gigayears. The global properties of FRB hosts are indistinguishable from core-collapse supernovae (CCSNe) and short gamma-ray bursts (SGRBs) hosts, and the spatial offset (from galaxy centers) of FRBs is mostly inconsistent with that of the Galactic neutron star population (95% confidence). The spatial offsets of FRBs (normalized to the galaxy effective radius) also differ from those of globular clusters (GCs) in late- and early-type galaxies with 95% confidence.

==> FRB host population/tables/AllFRBsprop.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
%\startlongtable

\begin{deluxetable*}{cccccccccccc}

\tablewidth{0pc}
\tablecaption{Host galaxies of six repeating and ten non-repeating FRBs used in this work, for which PATH posterior probability is $>90\%$. Derived measurements for new FRB hosts are highlighted in cyan. Updated measurement of previously reported hosts in \citet{Heintz+20} are highlighted in gray. We have also added most probable host of FRB20171020A \citep{Mahony2018} in our sample including the published host of repeating FRB20200120E \citep{Bhardwaj+21} and FRB20201124A \citep{Fong+21}.
\label{tab:updated_properties}}
\tabletypesize{\footnotesize}

\tablehead{\colhead{S.No} &\colhead{FRB}  
& \colhead{z} & \colhead{Rep} 
& \colhead{Offset} 
& \colhead{R$_{\rm eff}$\tablenotemark{a}}
& \colhead{Mass}  
& \colhead{SFR} 
& \colhead{log(sSFR)} 
& \colhead{$M_{\rm r}$} &  \colhead{$u-r$} 
& \colhead{$Z$}  
\\
\colhead{} & \colhead{}
& \colhead{} & \colhead{} 
& \colhead{(kpc)} 
& \colhead{(kpc)}
& \colhead{(10$^{10}~M_{\odot}$)}  
& \colhead{($M_{\odot}$ yr$^{-1}$)} 
& \colhead{(yr$^{-1}$)} 
& \colhead{} &  \colhead{} 
&  \colhead{} 
\\
} 
\startdata 
1 &FRB20121102A & 0.1927 & y & $0.8 \pm0.1$ & $0.66\pm0.03$ & $0.01 \pm0.01$ & $0.15 \pm0.04$ & $-$8.99 & $-16.20 \pm0.08$ & $1.49 \pm0.18$  & 8.08  \\
\rowcolor{LightCyan}
2 & FRB20180301A & 0.3304 & y & $10.2 \pm3.0$ & $5.80 \pm 0.20$ & $0.23 \pm0.06$ & $1.93 \pm0.58$ & $-$9.08 & $-20.18 \pm0.07$ & $0.90 \pm0.11$  & 8.70  \\
3 & FRB20180916B & 0.0337 & y & $5.4 \pm0.0$ & $3.57\pm 0.36$& $0.22 \pm0.03$ & $0.06 \pm0.02$ & $-$10.58 & $-19.46 \pm0.05$ & $1.53 \pm0.06$  &  -  \\
4 & FRB20180924B & 0.3212 & n & $3.4 \pm0.8$ & $2.75\pm 0.10$ &$1.32 \pm0.51$ & $0.88 \pm0.26$ & $-$10.18 & $-20.81 \pm0.05$ & $1.78 \pm0.15$  & 8.93  \\
%5 & FRB20181112A & 0.4755 & n & $1.8 \pm34.9$& $7.19 \pm 1.70$ &$0.40 \pm0.20$ & $0.37 \pm0.11$ & $-$10.03 & $-20.40 \pm0.07$ & $1.12 \pm0.15$  & 8.86  \\
5 & FRB20190102C & 0.2912 & n & $2.3 \pm4.2$ & $4.43 \pm 0.51$ &$0.47 \pm0.54$ & $0.86 \pm0.26$ & $-$9.74 & $-19.87 \pm0.06$ & $1.44 \pm0.15$  & 8.70  \\
%\rowcolor{Gray}
%7 & FRB20190523A & 0.6600 & n & $27.2 \pm22.6$ & $3.28 \pm 0.18$ & $46.49 \pm35.51$ & $0.09 \pm0.03$ & $-$12.74 & $-22.69 \pm0.14$ & $2.20 \pm0.22$  &  -  \\
6 & FRB20190608B & 0.1178 & n & $6.5 \pm0.8$ & $2.84 \pm 0.23$ &$1.16 \pm0.28$ & $0.69 \pm0.21$ & $-$10.22 & $-21.22 \pm0.05$ & $1.40 \pm0.09$  & 8.85  \\
\rowcolor{Gray}
7 & FRB20190611B & 0.3778 & n & $11.7 \pm5.8$ & $2.15 \pm 0.11$ &$0.35 \pm0.70$ & $0.27 \pm0.08$ & $-$10.11 & $-19.29 \pm0.10$ & $1.29 \pm0.18$  & 8.71  \\
8 & FRB20190711A & 0.5220 & y & $1.6 \pm4.5$ & $2.94\pm 0.17$ &$ 0.08 \pm0.03$ & $0.42 \pm0.12$ & $-$9.29 & $-19.01 \pm0.08$ & $0.95 \pm0.16$  &  -  \\
\rowcolor{Gray}
9 & FRB20190714A & 0.2365 & n & $2.7 \pm1.8$ & $3.94\pm 0.05$ &$1.42 \pm0.55$ & $0.65 \pm0.20$ & $-$10.34 & $-20.37 \pm0.05$ & $1.51 \pm0.28$  & 9.03  \\
10 & FRB20191001A & 0.2340 & n & $11.1 \pm0.8$ & $5.55\pm 0.03$ & $4.64 \pm1.88$ & $8.06 \pm2.42$ & $-$9.76 & $-22.13 \pm0.05$ & $1.67 \pm0.19$  & 8.94  \\
\rowcolor{LightCyan}
11 & FRB20191228A & 0.2432 & n & $5.7 \pm3.3$ & $1.78 \pm 0.06$ & $0.54 \pm0.60$ & $0.50 \pm0.15$ & $-$10.03 & $-18.26 \pm0.05$ & $2.13 \pm0.74$  & 8.48 \\
\rowcolor{Gray}
12 & FRB20200430A & 0.1608 & n & $1.7 \pm2.2$ & $1.64 \pm 0.53$ & $0.21 \pm0.11$ & $0.26 \pm0.08$ & $-$9.89 & $-18.25 \pm0.05$ & $2.08 \pm0.30$  & 8.88  \\
\rowcolor{LightCyan}
13 & FRB20200906A & 0.3688 & n & $5.9 \pm2.0$ & $7.58 \pm 0.06$ & $1.33 \pm0.37$ & $0.48 \pm0.14$ & $-$10.44 & $-21.49 \pm0.05$ & $1.22 \pm0.11$  & 8.76  \\
14 & FRB20171020A\tablenotemark{*} & 0.0087 & n &  - & - & 0.09 & 0.13 & $-$9.84 & $-$17.9  & - & 8.30 \\
%16 & FRB20181030A & 0.0039 & y & - & 0.63 $\pm$0.22 & 0.38 $\pm$0.11 & $-$10.22 & $-$19.32 &- &  - &  - \\
15 & FRB20200120E\tablenotemark{*} & 0.0008 & y & $20.1 \pm3.0$ & 3.5 & $7.20 \pm1.70$ & $0.89 \pm0.27$ & $-$10.91 & $-$19.78  & $2.77 \pm0.00$ & - \\
16 & FRB20201124A\tablenotemark{*} & 0.0980 & y & $1.3\pm0.1$ & - & $1.70^{+0.08}_{-0.11}$ & $2.12^{+0.69}_{-0.28}$ & $-$9.90 & $-20.41 \pm0.03$ & $2.06 \pm0.55$  & 9.03 \\
\rowcolor{Gray}
-- &FRB20190523A & 0.6600 & n & $27.2 \pm22.6$ & $3.28 \pm 0.18$ & $46.49 \pm35.51$ & $0.09 \pm0.03$ & $-$12.74 & $-22.69 \pm0.14$ & $2.20 \pm0.22$  &  -  \\
\hline 
\enddata 
\tablenotetext{a}{Isophotal effective half-light radius are used for a sample of FRB host published in \citet{Mannings+20}. For remaining hosts, effective radius derived from \texttt{GALFIT} are used. }
\tablenotetext{*}{Host properties are taken from \citet{Mahony2018, Bhardwaj+21, Fong+21}. The observed magnitudes for FRB20171020A, FRB20200120E and FRB20201124A are approximated as rest-frame magnitudes because of their low redshifts. }
\end{deluxetable*} 


==> FRB host population/tables/FRB-functions.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
%\startlongtable
\begin{deluxetable}{ccccccccc}
\tablewidth{0pc}
\tablecaption{P-values for two-sample 1D-KS for comparing the mass-weighted stellar mass distributions (of all, star-forming (SF) and quiescent (Q) sample), star formation rate volume density distribution and the double exponential function for sSFRs of field galaxies with FRB host (repeating and non-repeating) cumulative mass, SFR and sSFR distribution.  \label{tab:pvalues_frbfunction}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{FRB Type} & \multicolumn{3}{c}{Stellar mass} & \colhead{SFR}  
& \colhead{sSFR} 
\\
\colhead{} & \colhead{All} & \colhead{SF} & \colhead{Q} & \colhead{All} & \colhead{SF} \\
} 
\startdata 
%FRB_Type & M & SFR & sSFR
All & 4e-6 & 0.002 & 4e-11 & 4e-4 & 5e-6 \\
Rep  & 0.014 & 0.029 & 6e-4 & 0.056 & 0.037 \\
Non-rep  & 7e-5 & 0.005 & 4e-8 & 0.001 & 7e-6 \\
\hline
\enddata 
\end{deluxetable} 

==> FRB host population/tables/Pvalues_transientsonly.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
%\startlongtable
\begin{deluxetable*}{cc|cccccc}
\tablewidth{0pc}
\tablecaption{P-values for two-sample 1D-KS after comparing the distributions of various properties (column 1) of the hosts of FRBs (all together and separated by repeating and on-off host population) with that of galaxies hosting ULXs, SGRBs, LGRBs, SLSNe, CCSNe and Type Ia SN. Highlighted cells shows the p-values ($>0.05$) for which the null hypothesis cannot be rejected. SGRBs and CCSNe remain as the
allowed dominant channels for
producing FRBs. \label{tab:pvalues}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{Property} & \colhead{FRB Type} &\colhead{}  
& \colhead{} & \colhead{Transients} 
& \colhead{} 
& \colhead{}  
& \colhead{}
\\
\colhead{} & \colhead{} &\colhead{ULXs}  
& \colhead{SGRBs} & \colhead{LGRBs} 
& \colhead{SLSNe} 
& \colhead{CCSNe}  
& \colhead{Type Ia}
\\
} 
\startdata 
% Prop & FRB_Type & ULX & SGRBs & LGRBs & SLSNe & CCSNe \\
Offset & Rep & \cellcolor{Gray}0.28 &\cellcolor{Gray}0.44 & \cellcolor{Gray}0.18 & \cellcolor{Gray}0.37 & \cellcolor{Gray}0.82 & \cellcolor{Gray}0.28\\
& Non-rep & \cellcolor{Gray}0.97 & \cellcolor{Gray}0.57 & 0.00 & 0.02 & \cellcolor{Gray}0.25 & \cellcolor{Gray}0.99 \\
 & All & \cellcolor{Gray}0.93 & \cellcolor{Gray}0.52 & 0.00 & 0.02 & \cellcolor{Gray}0.27 & \cellcolor{Gray}0.92\\
\hline
SFR & Rep & 0.01 & \cellcolor{Gray}0.93 & \cellcolor{Gray}0.96 & \cellcolor{Gray}0.86 & \cellcolor{Gray}0.65 & 0.03 \\
& Non-rep & 0.00 & \cellcolor{Gray}0.26 & \cellcolor{Gray}0.07 & \cellcolor{Gray}0.18 & 0.04 & 0.00\\
 & All & 0.00 & \cellcolor{Gray}0.68 & \cellcolor{Gray}0.23 & \cellcolor{Gray}0.44 & \cellcolor{Gray}0.15 & 0.00\\
\hline
log(M) & Rep & 0.00 & \cellcolor{Gray}0.36 & \cellcolor{Gray}0.29 & \cellcolor{Gray}0.06 & \cellcolor{Gray}0.73 & 0.02 \\
& Non-rep & 0.00 & \cellcolor{Gray}0.64 & 0.00 & 0.00 & \cellcolor{Gray}0.33 & 0.00 \\
& All & 0.00 & \cellcolor{Gray}0.59 & 0.00 & 0.00 & \cellcolor{Gray}0.50 & 0.00  \\
\hline
Z & Rep & - & \cellcolor{Gray}0.91 & - & - & - & -  \\
& Non-rep & - & \cellcolor{Gray}0.99 & - & - & - & -  \\
 & All & - & \cellcolor{Gray}0.84 & - & - & -& - \\
\hline
M$_{\rm r}$ & Rep & - & 0.01 & - & \cellcolor{Gray}0.06 & \cellcolor{Gray}0.36& -  \\
& Non-rep & - & \cellcolor{Gray}0.89 & - & 0.01 & \cellcolor{Gray}0.80& -  \\
 & All & - & \cellcolor{Gray}0.06 & - & 0.00 & \cellcolor{Gray}0.73& - \\
\hline
sSFR & Rep & \cellcolor{Gray}0.32 & \cellcolor{Gray}0.75 & \cellcolor{Gray}0.25 & 0.05 & \cellcolor{Gray}0.70 & \cellcolor{Gray}0.34  \\
& Non-rep & \cellcolor{Gray}0.46 & \cellcolor{Gray}0.08 &  0.00 & 0.00 & 0.00& 0.00  \\
& All & \cellcolor{Gray}0.42 & \cellcolor{Gray}0.39 & 0.00 & 0.00 & 0.01& 0.00 \\
\hline 
\enddata 
\end{deluxetable*} 

==> FRB host population/tables/frb_measurements.tex <==
\begin{deluxetable*}{lccc}
\tablewidth{0pc}
\tablecaption{Measured and derived properties of the new FRBs presented in this work. \label{tab:measurements}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{Properties}\tablenotemark{} & \colhead{FRB20180301A} &\colhead{FRB20191228A}  
& \colhead{FRB20200906A} 
\\
} 
\startdata 
         Arrival time\tablenotemark{a} (UT)  & 2020-05-28 19:14:47.310 & 2019-12-28 09:16:16.444 & 2020-09-06 21:40:50.923 \\
         S/N  & 19.0 \tablenotemark{b} & 22.9 & 19.2 \\
         DM (pc\,cm$^{-3}$) & $536^{+8}_{-13}$ & $297.5\pm 0.05$ & $577.8\pm 0.02$\\
         DM$_{\rm ISM}~\rm NE2001 $ (pc\,cm$^{-3}$) & 152 & 33 & 36\\
         DM$_{\rm ISM}~\rm YMW16 $ (pc\,cm$^{-3}$) & 254 & 20 & 38\\
         DM$_{\rm cosmic}$\tablenotemark{c} (pc\,cm$^{-3}$) & 289  & 210 & 324 \\
         RA (J2000) & 06h12m54.44s\,($\pm0.01\arcsec$$\pm0.62\arcsec$) & 22h57m43.30s\,($\pm0.34\arcsec$$\pm0.83\arcsec$)  & 03h33m59.08s\,($\pm0.10\arcsec$$\pm0.34\arcsec$) \\ 
         Dec (J2000) & +04d40$'$15.8\,($\pm0.01\arcsec$$\pm0.6\arcsec$) &  $-$29d35$'$38.7\,($\pm0.3\arcsec$$\pm0.8\arcsec$) & $-$14d$04'59.5$\,($\pm0.1\arcsec$$\pm0.6\arcsec$) \\
         Fluence (Jy\,ms) & $4.9^{+0.5}_{-0.4}$ & 40$^{+100}_{-40}$ & 59$^{+25}_{-10}$ \\
         Pulse width (ms)& $7^{+2}_{-3}$ & $2.3\pm 0.6$ \tablenotemark{d} & $6.0\pm 0.6$ \\
         %Rotation measure (RM) (rad~m$^{-2}$) &  \\
         Spectral energy density\tablenotemark{e} (erg\,Hz$^{-1}$)   & $6.9 \times 10^{30}$ & $6.4 \times 10^{31}$ & $1.1 \times 10^{32}$ \\
         Persistent source, & $<1.8\times 10^{22}$ & $<3.4\times 10^{21}$ & $<4.3\times 10^{21}$  \\
         radio luminosity (W\,Hz$^{-1}$) & 1.5\,GHz & 6.5\,GHz & 6\,GHz\\
         \\
         \textbf{Host galaxy} \\
        Redshift\tablenotemark{*} & 0.3304 & 0.2432 & 0.3688 \\
        %$u-r$ (restframe) & 0.9(1) & 2.1(7) & 1.22(11) \\
        $u-r$\tablenotemark{$\dagger$} (restframe) & $0.90 \pm0.11$ & $2.13 \pm0.74$ & $1.22\pm 0.11$ \\
        M$_{\rm r}$\tablenotemark{$\dagger$} (restframe) & $-20.18\pm 0.07$ & $-18.26\pm0.05$ &  $-21.49 \pm 0.05$ \\
        Galactic $E(B-V)$\tablenotemark{$\dagger$} & 0.46 & 0.02 & 0.05 \\
        M$_*$\tablenotemark{$\dagger$} ($10^{10}~M_\odot$) & $0.23\pm 0.06$ &$0.54\pm 0.60$ & $1.33 \pm 0.37$ \\
        SFR\tablenotemark{*} ($M_\odot$~yr$^{-1}$) & $1.93\pm0.58$ & $0.50\pm 0.15$& $0.48 \pm 0.14$\\
        log(sSFR) (yr$^{-1}$) & $-$9.08 & $-$10.03 & $-$10.44\\
        %Stellar age (Gyr) & 0.61 & 0.76 & 0.64 \\
        Metallicity\tablenotemark{f} \tablenotemark{*} & 8.70 & 8.48 & 8.76 \\
        Projected offset from galaxy center (kpc) & $10.8 \pm3.0$ & $5.7\pm3.3$ & $5.9\pm2.0$ \\
        Effective radius (kpc) & $5.80\pm 0.20$ &$1.78\pm0.06$  & $7.58 \pm 0.06$ \\
 \tableline
\enddata 
\tablenotetext{a}{Arrival time of a repeating burst from FRB20180301A source and one-off ASKAP/CRAFT FRBs.}
\tablenotetext{b}{This is the coherent S/N of the FRB detected in the VLA image.} 
\tablenotetext{c}{Estimated using the Macquart-relation.}
\tablenotetext{d}{FRB20191228A shows a scattering tail of $6.1(6)$~ms. The deconvolved width is $2.3(6)$~ms. }
\tablenotetext{e}{The energies are derived assuming a flat spectrum for FRBs ($\alpha=0$) and zero k-correction.}
\tablenotetext{f}{In units of 12 + log[O/H].}
\tablenotetext{*}{These measurements are derived from spectroscopy. }
\tablenotetext{\dagger}{These properties are derived using \texttt{CIGALE} SED fitting.}
\tablenotetext{}{1$\sigma$ uncertainties are quoted for these measurements.} 
\end{deluxetable*} 


\begin{comment}
\begin{table*}
    \begin{threeparttable}
    \begin{tabular}{lccc}
        \hline
         Properties\tnote{} & FRB20180301A & FRB20191228A & FRB20200906A \\
         \hline
         Arrival time\tnote{a} (UT)  & 2020-05-28 19:14:47.310 & 2019-12-28 09:16:16.444 & 2020-09-06 21:40:50.923 \\
         S/N  & 19.0 \tnote{b} & 22.9 & 19.2 \\
         DM (pc\,cm$^{-3}$) & $536^{+8}_{-13}$ & $297.5\pm 0.05$ & $577.8\pm 0.02$\\
         DM$_{\rm ISM}~\rm NE2001 $ (pc\,cm$^{-3}$) & 152 & 33 & 36\\
         DM$_{\rm ISM}~\rm YMW16 $ (pc\,cm$^{-3}$) & 254 & 20 & 38\\
         DM$_{\rm cosmic}$\tnote{c} (pc\,cm$^{-3}$) & 289  & 210 & 324 \\
         RA (J2000) & 06h12m54.42s\,$\pm0.01\arcsec$$\pm0.62\arcsec$ & 22h57m43.30\,$\pm0.34\arcsec$$\pm0.83\arcsec$  & 03h33m59.08\,$\pm0.01\arcsec$$\pm0.62\arcsec$ \\ 
         Dec (J2000) & +04d40$'$15.9\,$\pm0.10\arcsec$$\pm0.34\arcsec$ &  $-$29d35$'$38.7\,$\pm0.34\arcsec$$\pm0.82\arcsec$ & $-$14d$04'59.5$\,$\pm0.11\arcsec$$\pm0.55\arcsec$ \\
         Fluence (Jy\,ms) & $4.9^{+0.5}_{-0.4}$ & 40$^{+100}_{-40}$ & 59$^{+25}_{-10}$ \\
         Pulse width (ms)& $7^{+2}_{-3}$ & $2.3\pm 0.6$ \tnote{d} & $6.0\pm 0.6$ \\
         
         %Rotation measure (RM) (rad~m$^{-2}$) &  \\
         Spectral energy density\tnote{e} (erg\,Hz$^{-1}$)   & $6.9 \times 10^{30}$ & $6.4 \times 10^{31}$ & $1.1 \times 10^{32}$ \\
         Persistent source, & $<1.8\times 10^{22}$ & $<3.4\times 10^{21}$ & $<4.3\times 10^{21}$  \\
         radio luminosity (W\,Hz$^{-1}$) & 1.5\,GHz & 6.5\,GHz & 6\,GHz\\
         \\
         \textbf{Host galaxy} \\
        Redshift\tnote{*} & 0.3304 & 0.2432 & 0.3688 \\
        %$u-r$ (restframe) & 0.9(1) & 2.1(7) & 1.22(11) \\
        $u-r$\tnote{$\dagger$} (restframe) & $0.90 \pm0.11$ & $2.13 \pm0.74$ & $1.22\pm 0.11$ \\
        M$_{\rm r}$\tnote{$\dagger$} (restframe) & $-20.18\pm 0.07$ & $-18.26\pm0.05$ &  $-21.49 \pm 0.05$ \\
        Galactic $E(B-V)$\tnote{$\dagger$} & 0.46 & 0.02 & 0.05 \\
        M$_*$\tnote{$\dagger$} ($10^{10}~M_\odot$) & $0.23\pm 0.06$ &$0.54\pm 0.60$ & $1.33 \pm 0.37$ \\
        SFR\tnote{*} ($M_\odot$~yr$^{-1}$) & $1.93\pm0.58$ & $0.03\pm 0.01$& $0.48 \pm 0.14$\\
        log(sSFR) (yr$^{-1}$) & $-$9.08 & $-$11.28 & $-$10.44\\
        %Stellar age (Gyr) & 0.61 & 0.76 & 0.64 \\
        Metallicity\tnote{f} \tnote{*} & 8.70 & 8.48 & 8.76 \\
        Projected offset from galaxy center (kpc) & $10.8 \pm3.0$ & $5.7\pm3.3$ & $5.9\pm2.0$ \\
        Effective radius (kpc) & $5.80\pm 0.20$ &$1.78\pm0.06$  & $7.58 \pm 0.06$ \\
        \hline
      \end{tabular}
       \caption{Measured and derived properties of the new FRBs presented in this work. }
       \label{tab:measurements}
       \begin{tablenotes}
\item [a] Arrival time of a repeating burst from FRB20180301A source and one-off ASKAP/CRAFT FRBs.
\item [b]This is the coherent S/N of the FRB detected in the VLA image. 
\item [c] Estimated using the Macquart-relation.
\item [d] FRB20191228A shows a scattering tail of $6.1(6)$~ms. The deconvolved width is $2.3(6)$~ms. 
\item [e] The energies are derived assuming a flat spectrum for FRBs ($\alpha=0$) and zero k-correction.
\item [f] In units of 12 + log[O/H].
\item[*] These measurements are derived from spectroscopy. 
\item[$\dagger$] These properties are derived using \texttt{CIGALE} SED fitting.
\item[] 1$\sigma$ uncertainties are quoted for these measurements. 
\end{tablenotes}
\end{threeparttable}
\end{table*}
\end{comment}

==> FRB host population/tables/photometry.tex <==
\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
%\startlongtable

\begin{deluxetable*}{cccccccc}

\tablewidth{0pc}
\tablecaption{Photometric measurements for a sample of new FRBs in this work and updated Pan-STARRS measurements for old FRBs published in \citet{Heintz+20}. All photometry have been corrected for Galactic extinction. 
\label{tab:photometry}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{Filter} &\colhead{FRB20180301A}  
& \colhead{FRB20191228A} & \colhead{FRB20200906A} 
& \colhead{FRB20190523A} 
& \colhead{FRB20190611B} 
& \colhead{FRB20190714A}
& \colhead{FRB20200430A} \\
} 
\startdata 
NOT$_u$ & $21.46\pm0.30$ & - & - & - & - & - & - \\
NOT$_g$ & $21.40\pm0.09$ & - & - & - & - & - & -\\
NOT$_r$ & $21.04\pm0.06$ & - & - &- & - & - & -\\
NOT$_i$ & $20.99\pm0.06$ & - & - &- & - & - & -\\
NOT$_z$ & $20.59\pm0.11$ & - & - &- & - & - & -\\
Pan-STARRS$_g$ & - &  - & $20.93\pm0.05$ & $22.10\pm0.14$ & - & $20.88\pm0.04$ & $22.21\pm0.10$\\
Pan-STARRS$_r$ & - &  - & $20.15\pm0.03$ & $21.91\pm0.15$ & - & $20.32\pm0.03$ & $21.25\pm0.07$\\
Pan-STARRS$_i$ & - &  - & $19.89\pm0.02$ & $20.86\pm0.08$ & - & $19.82\pm0.02$ & $20.97\pm0.05$\\
Pan-STARRS$_z$ & - &  - & $19.62\pm0.03$ & $20.63\pm0.09$ & - & $19.63\pm0.03$ & $20.71\pm0.10$\\
Pan-STARRS$_y$ & - &  - & $19.65\pm0.08$ & $19.88\pm0.11$ & - & $19.43\pm0.06$ & -\\
VLT/FORS2$_g$ & - & $22.61\pm0.50$  & $20.54\pm0.05$ & - & $23.24 \pm 0.09$ & \citet{Heintz+20} & - \\
VLT/FORS2$_I$ & - & $21.96\pm0.40$  & $19.51\pm0.02$ & - & $22.02 \pm 0.07$ & \citet{Heintz+20} & - \\
MMT/MMRS$_J$ & $20.56\pm0.07$ & - & - &  - & - & - & -\\
MMT/MMRS$_H$ & $20.40\pm0.08$ & - & - & - & - & - & -\\
MMT/MMRS$_K$ & $20.51\pm0.08$ & - & - & - & - & - & -\\
WISE$_{\rm W1}$ & - & - & $16.65\pm0.07$  &  - & - & - & -\\
WISE$_{\rm W2}$ & - & - & $16.08\pm0.14$  &  - & - & - & -\\
WISE$_{\rm W3}$ & - & - & $12.42\pm0.49$  &  - & - & - & -\\
WISE$_{\rm W4}$ & - & - & $9.01$  &  - & - & - & -\\
\hline 
\enddata 
\end{deluxetable*} 

==> FRB host population/tables/spectrumtab.tex <==

\definecolor{LightCyan}{rgb}{0.88,1,1}
\definecolor{Gray}{gray}{0.9}
%\startlongtable
\begin{deluxetable*}{ccccc}
\tablewidth{0pc}
\tablecaption{Nebular line emission measurements in units of 10$^{-16}$~erg~s$^{-1}$~cm$^{-2}$. New FRB hosts presented in this paper are highlighted in cyan and old FRB hosts with new data are highlighted in gray. The data for FRB20171020A and FRB20201124A is taken from \citet{Mahony2018} and \citet{Fong+21} respectively. \label{tab:spectrum}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{FRB}  
& \colhead{$H\alpha$} & \colhead{$H\beta$} 
& \colhead{[N~{\sc ii}]} 
& \colhead{[O~{\sc iii}]}  
\\} 
\startdata 
FRB20121102A  &$2.61 \pm0.04$ &$0.96 \pm0.09$ &$<0.12$ &$4.38 \pm0.08$ \\
\rowcolor{LightCyan}
FRB20180301A  &$16.97 \pm0.18$ &$7.77 \pm0.61$ &$4.32 \pm0.32$ &$12.75 \pm0.65$ \\
FRB20180916B  &$40.27 \pm0.25$ &- &$15.24 \pm0.24$ &$71.62 \pm0.60$ \\
FRB20180924B  &$2.79 \pm0.03$ &$0.72 \pm0.02$ &$1.94 \pm0.03$ &$0.79 \pm0.02$ \\
%FRB20181112A  &$0.64 \pm0.08$ &$0.29 \pm0.02$ &$0.49 \pm0.10$ &$0.54 \pm0.03$ \\
FRB20190102C  &$5.66 \pm0.17$ &$1.90 \pm0.17$ &$1.69 \pm0.19$ &$3.80 \pm0.27$ \\
%FRB190523  &- $\pm$- &0.03 $\pm$-9990000000000000000.00 &- $\pm$- &- $\pm$- \\
FRB20190608B  &$27.65 \pm0.41$ &$8.37 \pm0.33$ &$18.32 \pm0.38$ &$14.95 \pm0.44$ \\
FRB20190611B  &$0.49 \pm0.05$ &$0.12 \pm0.03$ &$0.12 \pm0.04$ &$0.18 \pm0.04$ \\
FRB20190711A  &- &$0.26 \pm0.05$ &- &- \\
FRB20190714A  &$3.89 \pm0.03$ &$0.97 \pm0.03$ &$1.70 \pm0.03$ &$0.31 \pm0.03$ \\
FRB20191001A  &$27.38 \pm0.26$ &$5.01 \pm0.30$ &$13.91 \pm0.19$ &$3.62 \pm0.35$ \\
\rowcolor{LightCyan}
FRB20191228A  &$0.30 \pm0.02$ &$0.02 \pm0.02$ &$0.08 \pm0.02$ &$0.13 \pm0.03$ \\
\rowcolor{Gray}
FRB20200430A  &$4.27 \pm0.15$ &$1.15 \pm0.21$ &$2.02 \pm0.20$ &$1.17 \pm0.25$ \\
\rowcolor{LightCyan}
FRB20200906A  &$6.49 \pm0.07$ &$4.25 \pm0.14$ &$1.80 \pm0.06$ &$5.38 \pm0.17$ \\
FRB20201124A & 56.9$^{+14.9}_{-9.9}$ & 12.3$^{+3.0}_{-2.3}$ & 25.3$^{+6.0}_{-4.7}$ & 3.8$^{+2.1}_{-1.1}$ \\
%FRB20171020A & 
\hline 
\enddata 
\end{deluxetable*} 


==> FRB host population/tables/tab_frb_results.tex <==
%\startlongtable
\begin{deluxetable*}{cccccccccccccccc}
\tablewidth{0pc}
\tablecaption{Results for FRB Associations\label{tab:results}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{FRB}  
& \colhead{RA$_{\rm cand}$} & \colhead{Dec$_{\rm cand}$} 
& \colhead{$\theta$} 
& \colhead{\halflight}  
& \colhead{\gmag} 
& \colhead{Filter} & \colhead{\pchance} 
& \colhead{\PO} & \colhead{\POx} 
\\} 
\startdata 
FRB20121102A& 82.9945 & $33.1479$& 0.2& 0.28& 23.52& GMOS\_N\_i& 0.0039& 0.0245& 1.0000\\ 
FRB20180916A& 29.5012 & $65.7148$& 7.7& 3.03& 16.16& GMOS\_N\_r& 0.0005& 0.8200& 1.0000\\ 
FRB20180924B& 326.1054 & $-40.9002$& 0.8& 1.31& 21.32& VLT\_FORS2\_g& 0.0119& 0.8723& 0.9894\\ 
FRB20181112A& 327.3486 & $-52.9709$& 0.4& 0.67& 21.49& VLT\_FORS2\_I& 0.0622& 0.0784& 0.6678\\ 
FRB20190102C& 322.4149 & $-79.4756$& 0.5& 0.86& 20.73& VLT\_FORS2\_I& 0.0056& 0.8425& 1.0000\\ 
FRB20190523A& 207.0642 & $72.4706$& 3.4& 0.71& 22.13& LRIS\_R& 0.1158& 0.1974& 0.8154\\ 
FRB20190608B& 334.0203 & $-7.8988$& 2.5& 1.66& 17.60& VLT\_FORS2\_I& 0.0005& 0.9930& 1.0000\\ 
FRB20190611B& 320.7429 & $-79.3973$& 2.0& 0.50& 22.35& GMOS\_S\_i& 0.0407& 0.3322& 0.9741\\ 
FRB20190614D& 65.0743 & $73.7068$& 1.3& 0.41& 24.01& LRIS\_I& 0.0552& 0.1944& 0.5825\\ 
FRB20190711A& 329.4194 & $-80.3581$& 0.5& 0.46& 22.93& GMOS\_S\_i& 0.0172& 0.4782& 0.9937\\ 
FRB20190714A& 183.9795 & $-13.0212$& 1.2& 0.95& 19.48& VLT\_FORS2\_I& 0.0014& 0.7993& 1.0000\\ 
FRB20191001A& 323.3525 & $-54.7487$& 4.2& 1.36& 17.82& VLT\_FORS2\_I& 0.0010& 0.5075& 0.5980\\ 
FRB20200430A& 229.7064 & $12.3766$& 0.4& 0.72& 21.18& LRIS\_I& 0.0047& 0.9379& 1.0000\\ 
FRB20191228A& 344.4307 & $-29.5940$& 2.1& 0.49& 21.92& VLT\_FORS2\_I& 0.0251& 0.5596& 1.0000\\ 
FRB20200906A& 53.4958 & $-14.0833$& 1.6& 1.51& 20.70& VLT\_FORS2\_g& 0.0106& 0.8997& 1.0000\\ 
FRB20180301A& 93.2269 & $4.6704$& 2.3& 0.92& 22.07& GMOS\_S\_r& 0.0387& 0.7154& 0.9993\\ 
\hline 
\enddata 
\end{deluxetable*} 

